Beamformed Self-Interference Measurements at 28 GHz: Spatial Insights and Angular Spread

We present measurements and analysis of self-interference in multi-panel millimeter wave (mmWave) full-duplex communication systems at 28 GHz. In an anechoic chamber, we measure the self-interference power between the input of a transmitting phased array and the output of a colocated receiving phased array, each of which is electronically steered across a number of directions in azimuth and elevation. These self-interference power measurements shed light on the potential for a full-duplex communication system to successfully receive a desired signal while transmitting in-band. Our nearly 6.5 million measurements illustrate that more self-interference tends to be coupled when the transmitting and receiving phased arrays steer their beams toward one another but that slight shifts in steering direction (on the order of one degree) can lead to significant fluctuations in self-interference power. We analyze these measurements to characterize the spatial variability of self-interference to better quantify and statistically model this sensitivity. Our analyses and statistical results can be useful references when developing and evaluating mmWave full-duplex systems and motivate a variety of future topics including beam selection, beamforming codebook design, and self-interference channel modeling.

==> sec-biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo.pdf}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
%\begin{IEEEbiography}{Michael Shell}
%	Biography text here.
%\end{IEEEbiography}

% \vspace{5cm}

\section*{Biographies}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/ipr.jpg}}]{Ian~P.~Roberts}
    (Student Member, IEEE) received the B.S.~degree in electrical engineering from the Missouri University of Science and Technology and the M.S.~degree in electrical and computer engineering from the University of Texas at Austin.
    % He received his B.S. in electrical engineering from Missouri University of Science and Technology in 2018. 
    He is currently a Ph.D.~candidate at the University of Texas at Austin, where he is part of 6G@UT in the Wireless Networking and Communications Group. 
    He has industry experience developing and prototyping wireless technologies at AT\&T Labs, Amazon, GenXComm (startup), Sandia National Laboratories, and Dynetics, Inc.
    % His research interests are in the theory and implementation of millimeter wave communication, in-band full-duplex, and communication system optimization.
    His research interests are in the theory and implementation of millimeter wave systems, in-band full-duplex, and other next-generation technologies for wireless communication and sensing.
    % His research interests are in the theory, simulation, and implementation of next-generation technologies for wireless communication and sensing, with a focus on millimeter wave and terahertz systems for 5G and future 6G cellular communication.
    He is a National Science Foundation Graduate Research Fellow.
\end{IEEEbiography}%

% \vspace{-12cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/ac.jpg}}]{Aditya Chopra}
(Senior Member, IEEE) received the B.Tech degree in electrical engineering from the Indian Institute of Technology, Delhi, India, in 2006, and the M.S.~(2008) and Ph.D.~(2011) in electrical engineering from The University of Texas at Austin, Texas, USA. He has worked at Fastback Networks, National Instruments, and AT\&T Labs as a communication system engineer. In 2022 he joined Project Kuiper at Amazon as a Senior Communication Systems Engineer. His research interests include wireless physical layer optimization and prototyping of advanced wireless communication systems.
\end{IEEEbiography}%

% \vspace{-12cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/tn.jpg}}]{Thomas Novlan} 
(Member, IEEE) is a Principal Member of Technical Staff with the Advanced Wireless Technologies Group of AT\&T Labs based in Austin, Texas. He is currently working on air-interface research and standardization for 5G Advanced and 6G communication networks. He joined AT\&T in 2016, working on technologies such as Dynamic Spectrum Sharing (DSS) and Integrated Access and Backhaul (IAB). He received his B.S.~with High Honors, M.S., and Ph.D.~in Electrical Engineering from The University of Texas at Austin in 2007, 2009, and 2012 respectively.
\end{IEEEbiography}%

% \vspace{-11cm}

% \newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/sv.jpg}}]{Sriram~Vishwanath}
(Fellow, IEEE) received the B.Tech.~degree in Electrical Engineering from the Indian Institute of Technology (IIT), Madras, India, in 1998, the M.S.~degree in Electrical Engineering from California Institute of Technology (Caltech), Pasadena, CA, USA, in 1999, and the Ph.D.~degree in Electrical Engineering from Stanford University, Stanford, CA, USA, in 2003.
For the past 18 years, he has been a Professor of Electrical and Computer Engineering at The University of Texas at Austin.
    
Sriram's research is in the domains of wireless networking and systems, information and coding theory, machine learning systems, and blockchain systems. He has over 300 refereed research papers and multiple research awards. He works across a diverse set of areas and specializes in bridging the gap between theory and practice. In particular, he has been involved in multiple spinouts from The University of Texas (as well as startups independent from The University of Texas).
    
Sriram received the NSF CAREER award in 2005 and the ARO Young Investigator Award in 2008. He was the UT Faculty Entrepreneur of the Year in 2014. He is a Fellow of the IEEE.
\end{IEEEbiography}%

% \vspace{-9.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/jga.jpg}}]{Jeffrey~G.~Andrews}
(Fellow, IEEE) received the B.S.~in Engineering with High Distinction from Harvey Mudd College, and the M.S.~and Ph.D.~in Electrical Engineering from Stanford University.  He is the Cockrell Family Endowed Chair in Engineering at the University of Texas at Austin where he is Director of the 6G@UT research center. He developed CDMA systems at Qualcomm, and has served as a consultant to Samsung, Nokia, Qualcomm, Apple, Verizon, AT\&T, Intel, Microsoft, Sprint, and NASA. He is co-author of the books \textit{Fundamentals of WiMAX} (Prentice-Hall, 2007) and \textit{Fundamentals of LTE} (Prentice-Hall, 2010).  He was the Editor-in-Chief of the \textsc{IEEE Transactions on Wireless Communications} from 2014-2016, and is the founding Chair of the Steering Committee for the \textsc{IEEE Journal on Selected Areas in Information Theory} (2018-23), and the Chair of the {IEEE Communication Theory Technical Committee} (2021-22).  

Dr. Andrews is an IEEE Fellow and ISI Highly Cited Researcher and has been co-recipient of 15 best paper awards including the 2016 IEEE Communications Society \& Information Theory Society Joint Paper Award, the 2014 IEEE Stephen O.~Rice Prize, the 2014 and 2018 IEEE Leonard G.~Abraham Prize, the 2011 and 2016 IEEE Heinrich Hertz Prize, and the 2010 IEEE ComSoc Best Tutorial Paper Award.  His other major awards include the 2015 Terman Award, the NSF CAREER Award, the 2021 Gordon Lepley Memorial Teaching Award at UT Austin, the 2021 IEEE ComSoc Joe LoCicero Service Award, the 2019 IEEE Wireless Communications Technical Committee Recognition Award, and the 2019 IEEE Kiyo Tomiyasu technical field award.
\end{IEEEbiography}%


% \vspace{-12cm}




==> sec-keywords.tex <==
\begin{keywords}
Millimeter-wave
\end{keywords}

==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle
